ILP Modulo Data

The vast quantity of data generated and captured every day has led to a pressing need for tools and processes to organize, analyze and interrelate this data. Automated reasoning and optimization tools with inherent support for data could enable advancements in a variety of contexts, from data-backed decision making to data-intensive scientific research. To this end, we introduce a decidable logic aimed at database analysis. Our logic extends quantifier-free Linear Integer Arithmetic with operators from Relational Algebra, like selection and cross product. We provide a scalable decision procedure that is based on the BC(T) architecture for ILP Modulo Theories. Our decision procedure makes use of database techniques. We also experimentally evaluate our approach, and discuss potential applications.

==> reviews <==
----------------------- REVIEW 1 ---------------------
PAPER: 79
TITLE: ILP Modulo Data
AUTHORS: Panagiotis Manolios, Vasilis Papavasileiou and Mirek Riedewald


----------- REVIEW -----------
This paper combines an ILP solver with a theory of database tables
(relations in extension). This is done in ILP modulo theories
framework in which an ILP solver takes the role of the SAT solver in a
lazy SMT solver. The tuples in the relations can derive from a
concrete database, or they can be symbolic (contain variables). The
paper defines a logic called Delta that incorporates linear arithmetic
and operations on relations. Satisfiability in the combined theories
can be decided by reduction to LIA. This reduction is polynomial for
fixed nesting depth of relational operators, but the exponent
increases with depth (specifically of the relational cross product
operator).

The paper focuses on an alternative approach (for existential formulas)
that uses an NO-style combination. There is a dedicated solver for the
tuple inclusion relation that can propagate constraints and propose
branching predicates based on data in the tables. This is shown using
some generated benchmark problems to be much more efficient than using
the eager reduction, either with an ILP-based solver or with Z3.

It is also suggested that the solver could be integrated with a
traditional DBMS to exploit its query optimization capabilities,
though this idea is not worked out in much detail in the paper.

The general concept and the combination framework are fairly well
described. However, the actual methods of propagation and branching
are described mainly by examples. The general idea is there, but it is
hard to know what is actually implemented.

One interesting aspect of the procedure is that, while the two
theories are disjoint, the relational theory nonetheless propagates
inequalities based on numeric values in the tables. This is not needed
for completeness, but contributes to efficient search (in fact, this
seems to be the main idea that gives better efficiency than eager
reduction).

It also fits neatly within the BC(T) framework. Still, it is not clear
why the same could not be done in a DPLL(T) framework. The paper seems
to take it for granted that the ILP approach will be more efficient
and does not consider the other possibility. Some motivation for this
choice would be helpful (or even better an experimental comparison,
though obviously this is not a small project).

Three example applications are given: generating test data, finding a
rectangle containing N geographic points, and picking a stock
portfolio to maximize historic return. Constraint-based test
generation is used in practice in hardware testing, so perhaps this is
a connection to CAD (perhaps we can imagine a database of packets to
be transmitted with variable fields to be filled in?). For the other
two problems, we might imagine writing a custom branch-and-bound
solver, but the paper's method lets us use a generic solver. While
the problems themselves are perhaps not of great interest, they
suggest a broader range of applications.

The paper uses the buzz phrase "big data" a bit recklessly. The method
doesn't really apply to big data (if by this we mean data that is
"big" even for a traditional DBMS). It would be better to say that it
gives a richer query language for small data, allowing analyses for
which we might otherwise have to write custom solvers.

Overall, though the connection to CAD is tenuous, the work is original
and I think the concepts would be interesting to the FMCAD audience.

----------------------- REVIEW 2 ---------------------
PAPER: 79
TITLE: ILP Modulo Data
AUTHORS: Panagiotis Manolios, Vasilis Papavasileiou and Mirek Riedewald


----------- REVIEW -----------
This paper introduces a framework (and logic) for symbolic reasoning about databases.  The logic (\Delta-logic) is an extension of QFIA with database tables.  In addition, the authors provide a procedure (ILP modulo data) which is essentially a Nelson-Oppen combination of ILP solver with database techniques.

This is a good paper, providing interesting new application to formal reasoning techniques. Although the application is not particularly deep (e.g., providing a logic and decision procedure by the obvious combination of ILA and database operations), I do applaud the authors' efforts to use formal methods beyond its traditional target zones.  The paper also does a good job of explaining the logic features with motivating examples. 

One area where the paper lacks a bit is related work.  In particular, I believe a bit more comparison with [17] and [8] is warranted.  In particular, I believe [8] has a very similar approach, although admittedly with a general-purpose solver.  The statement "We are not aware of available tools stemming from the research mentioned" is probably provided as a reason for not doing more thorough comparison.  Nevertheless, the papers themselves do provide information/applications of the approaches and I believe a better comparison is possible.  Or perhaps the authors think that the comparison between Inez and InezDB provides an analogy because Inez is more generic.  Whatever it is, must be clarified.

I personally did not see much value in the complexity results (Theorems 1-4), --- they seem to be rather obvious reductions.  So I will much rather prefer a more thorough comparison with related work than these theorems and their proofs, if space is an issue.

Minor comments: 

In some spots, particularly Section V A, the fonts are small, perhaps because of a latex font specification problem.

----------------------- REVIEW 3 ---------------------
PAPER: 79
TITLE: ILP Modulo Data
AUTHORS: Panagiotis Manolios, Vasilis Papavasileiou and Mirek Riedewald


----------- REVIEW -----------
This paper introduces a logic and solver architecture for integrating
constraint solvers (in particular ILP) with relational databases; the
goal is to develop tools that can perform complex reasoning and
optimisation on data sets that are too large to be handled by existing
solvers or theorem provers. After motivation, the paper first defines
the logic Delta, which augments QFLIA with syntax and operators for
working with finite tables of (concrete or symbolic) data, and
examines the complexity of important fragments. Delta formulae can be
reduced to QFLIA, but at the cost of potentially exponential growth in
size. Focusing on the existential fragment of Delta, the authors then
develop a modular solver architecture in which an ILP system takes
care of arithmetic constraints, while a database system reasons about
table membership. The two "solvers" cooperate Nelson-Oppen-style by
exchanging implied equalities; in addition, bound propagation is used
to reduce the amount of branching necessary. Experiments show that the
resulting solver outperforms the SMT solver Z3, as well as the
ILP/BC(T)-based system Inez (without database support), for relevant
applications with substantial amount of represented data.

Comments:

The paper presents a very elegant and thorough approach to constraint
solving in the context of large data collections. The problem is well
motivated, and clearly relevant in areas overlapping with the scope of
FMCAD. The solution is developed systematically starting from the
logic Delta, design and implementation details are discussed on a
reasonable level, and experiments are convincing.

While theoretically elegant, I am wondering whether the use of
Nelson-Oppen for combining membership constraints with other theories
(here, integers) is overkill. As the authors observe in the appendix,
table memberships are (conceptually) really short-hand notation for
disjunctions of (vector) equations, so they don't form an interesting
theory on their own. In fact, Lemma 2 should hold even for theories T
that are not stably infinite?

The paper gives little information on how the procedure can be
extended to support optimisation; a few sentences on this would be
interesting.

p3: I don't see how the "count" aggregate function can naturally be
expressed (though I wouldn't be surprised if this is possible)

p4: "eager scheme" should that be "lazy"?

----------------------- REVIEW 4 ---------------------
PAPER: 79
TITLE: ILP Modulo Data
AUTHORS: Panagiotis Manolios, Vasilis Papavasileiou and Mirek Riedewald


----------- REVIEW -----------
Summary
========

The paper instantiates the framework of "ILP Modulo Theories" to the
case of a "theory of data", which is intended to model the state of a
data base.

The paper introduces a decidable logic that extends quantifier
free linear integer arithmetic with database tables and operators
from relational algebra (selection, union and cross product). It
also discusses complexity and decidability results of the
proposed logic.

The authors also identify a subset of the logic for which a
(scalable?) procedure based on the Branch & Cut(T) architecture for
ILP Modulo Theories is provided. 

The paper outlines potential application for the logic, provides an
experimental setup based on the collection of benchmarks from several
areas, and experimentally evaluate the approach.


Review
======

Significance:

The paper addresses an interesting problem, and proposes a complete
instantiation of ILP approach. In particular, it introduces a logic
for relational algebra with QFLIA, for which decidability and
complexity results are given, reduces the problem to the Branch &
Cut(T) architecture for ILP Modulo Theories, and demonstrates the
technique in a new application area (analysis of big data).


Originality:

Although the paper builds within the previously published ILP(T)
framework, there seems to be several original contributions: the
definition of the logic, its decidability and complexity results,
examples of encodings into ILP(data). However, a detailed related work
is missing - other relevant papers are only mentioned, without a clear
analysis of differences. In particular, reference [17] seems very
related and should be discussed in greater depth.

The authors should also discuss what is the role of ILP(T) in this
setting: would DPLL(data) be as strong as ILP(data)? The experimental
comparison agains Z3 does not answer this question. What it does is to
compare the ILP(data) with an encoding of the same problem into
SMT(QF_LIA). The proposed approach relies on a dedicated solver for
the data theory. In principle, it should be possible to embed the
solver for the theory of data directly into an DPLL(T)
architecture. In the current setting it is hard to assess the merits
of the dedicate solver vs the merit of ILP(T) compared to DPLL(T).  If
the key difference is in the ability to carry out optimization, which
can be encoded within SMT only indirectly, this should be stated
explicitly (in which case the comparison with Z3 should be described
in greater detail).

Experimental evaluation:

The authors claim that the proposed decision procedure is "scalable;
however, little evidence of scalability is provided in the
experiments.  This also impacts the claim of applicability of this
technique to big data, given that the biggest benchmark contains
"only" 640,000 tuples (which for a typical data base size is not an
impressive figure).

Quality of Presentation:

The paper is reasonably well written and organized. The technical
quality of the proofs is fair. Some minor comments are listed below.

Overall Evaluation:

On the positive side, the paper provides a demonstration of the the
use of symbolic reasoning with concrete data, introduces a new logic
with complexity and decidability results.

On the negative side, a detailed related work is missing, and the
experimental analysis could be improved.


Organization:
- In section III, it does not say anything about the equality
  when introducing the logic
- Figure 2 that gives rules of the grammar, is not comprehensive
  enough. A formula can be inequality between two terms, and a
  term can be a pair of terms. The following is possible
   (T_1, T_2) <= (T_3, T_4)
  and in the text, the authors restrict
  the inequality operation on the integer terms. Good point is
  that they have mentioned in the text.  This logic could have
  been better explained with multi-sorted logic.
- Definition1 and Theorem3 seems unnecessary.
- used the notion of constraints before defining it. (used in
  example 1 and defined it in definition3)
- it talks about T-satisfiability without defining it or
  providing the reader the reference.
- related work is not discussed in detail. Reference [17] seems
  very related.

